Ant Colony Sampling with GFlowNets for Combinatorial Optimization

We present the Generative Flow Ant Colony Sampler (GFACS), a novel meta-heuristic method that hierarchically combines amortized inference and parallel stochastic search. Our method first leverages Generative Flow Networks (GFlowNets) to amortize a \emph{multi-modal} prior distribution over combinatorial solution space that encompasses both high-reward and diversified solutions. This prior is iteratively updated via parallel stochastic search in the spirit of Ant Colony Optimization (ACO), leading to the posterior distribution that generates near-optimal solutions. Extensive experiments across seven combinatorial optimization problems demonstrate GFACS's promising performances.

==> tables/cvrp_nls.tex <==
\begin{tabular}{lccccccccc}
\toprule[1.0pt]
\multicolumn{1}{c}{} & \multicolumn{3}{c}{CVRP200} & \multicolumn{3}{c}{CVRP500} &
\multicolumn{3}{c}{CVRP1000} 
\\ 
\cmidrule[0.5pt](lr{0.2em}){2-4}
\cmidrule[0.5pt](lr{0.2em}){5-7}
\cmidrule[0.5pt](lr{0.2em}){8-10}
Method
 & Obj. & Gap(\%)
 & Time & Obj. & Gap(\%) & Time
 & Obj. & Gap(\%) & Time 
\\ 
\midrule[1.0pt]
PyVRP & 27.93 & 0.00 & 4.0m & 62.96 & 0.00 & 21.0m & 119.29 & 0.00 & 1.4h \\ 
LKH-3 & 28.02 & 0.30 & 2.4m & 63.07 & 0.18 & 18.6m & 119.52 & 0.20 & 2.1h 
\\
\cmidrule(lr{0.1em}){1-1}
\cmidrule(lr{0.1em}){2-4}
\cmidrule(lr{0.1em}){5-7}
\cmidrule(lr{0.1em}){8-10}
%POMO+AS{*} {[}{]} & - & - & - & - & - & - & - & - & - 
%\\
POMO & 29.12 & 4.25 & 1s & 68.69 & 9.08 & 2s & 145.74 & 22.14 & 3s
\\
POMO + EAS & \textbf{27.99} & \textbf{0.20} & 2.0m & 64.76 & 2.85 & 5.0m & 126.25 & 5.83 & 10.0m
\\
POMO + SGBS & 28.07 & 0.49 & 2.0m & 65.44 & 3.93 & 5.2m & 127.90 & 7.21 & 10.1m  
% \\
% POMO+MetaSAGE{*} {[}{]}  & - & - & - & 63.32 & 0.04 & - & - & - & -
% %Sym-NCO+AS{*} {[}{]}  & - & - & - & - & - & - & - & - & - 
\\
SymNCO  & 29.15 & 4.34 & 1s & 68.81 & 9.28 & 2s & 141.82 & 18.86 & 3s 
\\
SymNCO + EAS & 28.01 & 0.58 & 2.0m & 64.63 & 2.65 & 5.0m & 125.58 & 5.27 & 10.0m 
\\
SymNCO + SGBS  & 28.10 & 0.61 & 2.0m & 65.40 & 3.87 & 5.2m & 127.53 & 6.90 & 10.1m 
\\
\cmidrule(lr{0.1em}){1-1}
\cmidrule(lr{0.1em}){2-4}
\cmidrule(lr{0.1em}){5-7}
\cmidrule(lr{0.1em}){8-10}
ACO {$(T = 10)$} & 28.45 & 1.86 & 13s & 64.62 & 2.63 & 36s & 122.82 & 2.96 & 1.3m 
\\
DeepACO {$(T = 10)$} & 28.44 & 1.80 & 14s & 64.49 & 2.43 & 36s & 122.15 & 2.40 & 1.3m
\\
GFACS {$(T = 10)$} & 28.32 & 1.40 & 14s & \textbf{64.19} & \textbf{1.95} & 36s & \textbf{121.80} & \textbf{2.11} & 1.3m
\\
%DeepACO {$(T = 2)$} & - & - & - & - & - & - & - & - & - 
%\\
%Ours {$(T = 2)$} & - & - & - & - & - & - & - & - & - 
%\\ 
%DeepACO {$(T = 10)$} & - & - & - & - & - & - & - & - & - 
%\\ 
%Ours {$(T = 10)$} & - & - & - & - & - & - & - & - & - 
%\\
%DeepACO {$(T = 100)$} & - & - & - & - & - & - & - & - & - 
%\\ 
%Ours {$(T = 100)$} & - & - & - & - & - & - & - & - & - 
%\\
\bottomrule[1.0pt]
\end{tabular}


==> tables/tsp_nls.tex <==
\begin{tabular}{lccccccccc}
\toprule[1.0pt]
 & \multicolumn{3}{c}{TSP200} & \multicolumn{3}{c}{TSP500} & \multicolumn{3}{c}{TSP1000} 
\\ 
\cmidrule[0.5pt](lr{0.2em}){2-4}
\cmidrule[0.5pt](lr{0.2em}){5-7}
\cmidrule[0.5pt](lr{0.2em}){8-10}
Method & Obj. & Gap(\%)
 & Time(s) & Obj. & Gap(\%) & Times(s)
 & Obj. & Gap(\%) & Time(s) 
\\ 
\midrule[1.0pt]
Concorde & 10.72 & 0.00 & 0.9 & 16.55 & 0.00 & 10.7 & 23.12 & 0.00 & 108 
\\
LKH-3 & 10.72 & 0.00 & 9.8 & 16.55 & 0.02 & 31.7 & 23.14 & 0.10 & 102 
\\
\cmidrule(lr{0.1em}){1-1}
\cmidrule(lr{0.1em}){2-4}
\cmidrule(lr{0.1em}){5-7}
\cmidrule(lr{0.1em}){8-10}
AM{*} & 12.00 & 11.91 & 0.2 & 21.46 & 29.07 & 0.6 & 33.55 & 45.10 & 1.5 
\\
POMO{*} & 10.89 & 1.62 & 0.1 & 20.57 & 24.40 & 0.6 & 32.90 & 42.30 & 4.1 

\\
POMO + EAS & 10.75 & 0.30 & 120 & 18.25 & 10.29 & 300 & 30.77 & 33.06 & 600
\\
POMO + SGBS & 10.77 & 0.43 & 133 & 18.86 & 13.98 & 318 & 28.58 & 23.61 & 605 
\\
%GCN+MCTS{*} {[}{]} & 10.81 & 0.88 & 149.6 & 16.97 & 2.54 & 50 & 23.86 & 3.22 & 100 
%\\
DIMES + MCTS{*} & - & - & - & 17.01 & 2.78 & 11 & 24.45 & 5.75 & 32 
\\
%DIFUSCO+MCTS{*} {[}{]} & - & - & - & 16.63 & 0.46 & 4.7 & 23.39 & 1.17 & 11 
%\\
SO{*} & 10.78 & 0.63 & 10 & 16.94 & 2.40 & 15 & 23.77 & 2.80 & 26 
\\
Pointerformer{*} & 10.79 & 0.68 & 5.5 & 17.14 & 3.56 & 14 & 24.80 & 7.90 & 40 
\\
H-TSP{*} & - & - & - & - & - & - & 24.65 & 6.62 & 0.3 
\\
\cmidrule(lr{0.1em}){1-1}
\cmidrule(lr{0.1em}){2-4}
\cmidrule(lr{0.1em}){5-7}
\cmidrule(lr{0.1em}){8-10}
ACO {$(T = 10)$} & 10.91 & 1.77 & 2.1 & 17.38 & 5.04 & 14 & 24.76 & 7.09 & 57 
\\
DeepACO {$(T = 10)$} & 10.77 & 0.45 & 2.5 & 16.84 & 1.77 & 15 & 23.78 & 2.87 & 66
\\ 
GFACS {$(T = 10)$} & \textbf{10.75} & \textbf{0.26} & 2.5 & \textbf{16.80} & \textbf{1.56} & 15 & \textbf{23.72} & \textbf{2.63} & 66
\\
%DeepACO {$(T = 2)$} & 10.82 & 0.97 & - & 16.94 & 2.36 & 2.0 & 23.99 & 3.76 & 6.4
%\\
%Ours {$(T = 2)$} & 10.77 & 0.49 & - & - & - & -
%\\ 
%DeepACO {$(T = 10)$} & 10.78 & 0.57 & 2.4 & 16.86 & 1.84 & 10 & 23.85 & 3.16 & 32
%\\ 
%Ours {$(T = 10)$} & 10.75 & 0.26 & 2.5 & - & - & -
%\\
%DeepACO {$(T = 100)$} & - & - & - & - & - & - & - & - & - 
%\\ 
%Ours {$(T = 100)$} & - & - & - & - & - & - & - & - & - 
%\\
\bottomrule[1.0pt]
\end{tabular}


==> tables/vsVarGrad.tex <==
\begin{tabular}{lcccc}
\toprule[1.0pt]
\multicolumn{1}{c}{} & \multicolumn{2}{c}{TSP500} & \multicolumn{2}{c}{CVRP500}\\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
% \cmidrule[0.5pt](lr{0.2em}){2-3}
% \cmidrule[0.5pt](lr{0.2em}){4-5}
% \cmidrule[0.5pt](lr{0.2em}){6-7}
% \cmidrule[0.5pt](lr{0.2em}){8-9}
\
Method & Obj. & Gap (\%) & Obj. & Gap (\%) \\
\midrule
Concorde / PyVRP & 16.55 & - & 62.96 & - \\
\midrule
GFACS w/ \textit{VarGrad} ($T=10$) & 16.86 & 1.88 & 64.28 & 2.09 \\
GFACS w/ \textit{Shared $\varepsilon$-norm} ($T=10$) & \textbf{16.80} & \textbf{1.56} & \textbf{64.19} & \textbf{1.95} \\
\bottomrule
\end{tabular}
